Joint Recognition of Handwritten Text and Named Entities with a Neural End-to-end Model

When extracting information from handwritten documents, text transcription and named entity recognition are usually faced as separate subsequent tasks. This has the disadvantage that errors in the first module affect heavily the performance of the second module. In this work we propose to do both tasks jointly, using a single neural network with a common architecture used for plain text recognition. Experimentally, the work has been tested on a collection of historical marriage records. Results of experiments are presented to show the effect on the performance for different configurations: different ways of encoding the information, doing or not transfer learning and processing at text line or multi-line region level. The results are comparable to state of the art reported in the ICDAR 2017 Information Extraction competition, even though the proposed technique does not use any dictionaries, language modeling or post processing.

==> Makefile <==
NAME=main
BIBTEX=yes
#PDFOPTIM=yes
PDFOPTIMOPTIONS=--gs --web

pdflatex:
	${MAKE} TYPE=pdflatex all

latex:
	${MAKE} TYPE=latex all

all: ${NAME}.pdf

ifeq (${TYPE},latex)

${NAME}.pdf: ${NAME}.dvi
	dvipdf ${NAME}
ifeq (${PDFOPTIM},yes)
	pdfoptim.sh ${PDFOPTIMOPTIONS} --inplace ${NAME}.pdf
endif

ifeq (${BIBTEX},yes)
#${NAME}.dvi: ${NAME}*.tex ../tables/*.tex ../figures/*.tex ${NAME}.aux ${NAME}.bbl ${NAME}.blg
${NAME}.dvi: ${NAME}*.tex ${NAME}.aux ${NAME}.bbl ${NAME}.blg
	latex ${NAME}
else
#${NAME}.dvi: ${NAME}*.tex ../tables/*.tex ../figures/*.tex ${NAME}.aux
${NAME}.dvi: ${NAME}*.tex ${NAME}.aux
endif
	latex ${NAME}
#	latex ${NAME}

ifeq (${BIBTEX},yes)
${NAME}.aux: sample.bib
else
${NAME}.aux:
endif
	latex ${NAME}

else

ifeq (${BIBTEX},yes)
#${NAME}.pdf: ${NAME}*.tex ../tables/*.tex ../figures/*.tex ${NAME}.aux ${NAME}.bbl ${NAME}.blg
${NAME}.pdf: ${NAME}*.tex ${NAME}.aux ${NAME}.bbl ${NAME}.blg
	pdflatex -interaction=nonstopmode -halt-on-error ${NAME} #|| true
else
#${NAME}.pdf: ${NAME}*.tex ../tables/*.tex ../figures/*.tex ${NAME}.aux
${NAME}.pdf: ${NAME}*.tex ${NAME}.aux
endif
	pdflatex -interaction=nonstopmode -halt-on-error ${NAME} #|| true
	pdflatex -interaction=nonstopmode -halt-on-error ${NAME} #|| true
ifeq (${PDFOPTIM},yes)
	pdfoptim.sh ${PDFOPTIMOPTIONS} --inplace ${NAME}.pdf
endif

ifeq (${BIBTEX},yes)
${NAME}.aux: sample.bib
else
${NAME}.aux:
endif
	pdflatex -interaction=nonstopmode -halt-on-error ${NAME} #|| true

endif

bib:
	rm -f sample.bib ../bib/*.bib
	./findbibs.sh
	${MAKE} sample.bib

sample.bib:
	cat ../bib/*.bib | sed 's|\(^[ \t]*\)doi\([ \t]*=[ \t]*{\)\([^}]*\)\(.*\)|@@@@{\3}\4\n\1note\2doi:\\href{http://dx.doi.org/\3}|' | sed '/^@@@@/{ s|_|\\_|g; N; s|@@@@\([^\n]*\)\n\(.*\)|\2\1|; }' > sample.bib

${NAME}.bbl ${NAME}.blg: sample.bib
	bibtex ${NAME}

clean:
	rm -f ${NAME}.dvi ${NAME}.pdf

realclean: clean
	rm -f ${NAME}.aux ${NAME}.log ${NAME}.bbl ${NAME}.blg ${NAME}.brf ${NAME}.toc ${NAME}.out ${NAME}.idx

